Automatically Securing Permission-Based Software by Reducing the Attack Surface: An Application to Android

A common security architecture, called the permission-based security model (used e.g. in Android and Blackberry), entails intrinsic risks. For instance, applications can be granted more permissions than they actually need, what we call a "permission gap". Malware can leverage the unused permissions for achieving their malicious goals, for instance using code injection. In this paper, we present an approach to detecting permission gaps using static analysis. Our prototype implementation in the context of Android shows that the static analysis must take into account a significant amount of platform-specific knowledge. Using our tool on two datasets of Android applications, we found out that a non negligible part of applications suffers from permission gaps, i.e. does not use all the permissions they declare.

==> figures/android-framework-application-graph.tex <==
%% Framework Application Graph

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}
\tikzstyle{block} = [draw,fill=white!20,minimum width=4em]
\begin{tikzpicture}
  [node distance=.5cm,
  start chain=going below,]

		  \tikzstyle{vertex}=[circle,fill=black!25,minimum size=14pt,inner sep=0pt]
		  \tikzstyle{vInterface}=[block,fill=black!25,minimum size=14pt,inner sep=0pt]
  		\tikzstyle{tuborg}=[decorate]
  		\tikzstyle{tubnode}=[midway, right=2pt]
			% application nodes
		  \foreach \name/\x/\y in {s/1/0, 2/0/1, 3/1/1, 4/2/1, 5/1/2}
		    \node[vertex] (G-\name) at (\x,-\y/1.2) {$\name$};
			% interface nodes
		  \node[vInterface] (G-e1) at (0,-3/1.2) {$e_{1}$};
		  \node[vInterface] (G-e2) at (1,-3/1.2) {$e_{2}$};
		  \node[vInterface] (G-e3) at (2,-3/1.2) {$e_{3}$};
		  \node[vInterface] (G-idots) at (3,-3/1.2) {$...$};
		  \node[vInterface] (G-in) at (4,-3/1.2) {$e_L$};
		  \foreach \from/\to in {s/2, s/3, s/e3, 2/e1, 2/3, 3/5, 3/4, 5/2, 5/4, 5/e2}
		    \draw[->] (G-\from) -- (G-\to);
			% framework nodes
		  \foreach \name/\x/\y in {f1/0/4, f2/1/4, f3/2/4, f4/0/5, f5/1/5, f6/0/6, f8/4/4, f9/4/5}
		    \node[vertex] (G-\name) at (\x,-\y/1.2) {$\name$};
		  \foreach \name/\x/\y/\n in {ck/1/6/1, ck/3/5/2}
		    \node[vertex,fill=white] (G-\name\n) at (\x,-\y/1.2) {$\name_\n$};
		  \foreach \from/\to in {e1/f1, e2/f2, e3/f3, f1/f4, f2/f5, f2/f4, f4/f6, f4/ck1, f8/f9, f8/ck2, in/f8} 
		    \draw[->] (G-\from) -- (G-\to);

			% background
		  \node[] (G-00) at (0,0) {};
		  \node[] (G-10) at (2,0) {};
		  \node[] (G-01) at (0,-3/1.2) {};
		  \node[] (G-11) at (2,-3/1.2) {};
		  
			\node[] (G-F00) at (0,-3/1.2) {};
		  \node[] (G-F10) at (4,-3/1.2) {};
		  \node[] (G-F01) at (0,-6/1.2) {};
		  \node[] (G-F11) at (4,-6/1.2) {};
\begin{pgfonlayer}{background}
        % Compute a few helper coordinates
        \path (G-00.west |- G-10.north)+(-0.5,0.3) node (a) {};
        \path (G-01.north -| G-11.east)+(+0.3,-0.1) node (b) {};
        \path[fill=black!5,rounded corners, draw=black!50, dashed]
            (a) rectangle (b);
        \path (G-F00.west |- G-F10.south)+(-0.5,0.1) node (a) {};
        \path (G-F01.south -| G-F11.east)+(+0.3,-0.2) node (b) {};
        \path[fill=black!10,rounded corners, draw=black!50, dashed]
            (a) rectangle (b);
\end{pgfonlayer}

			% naming
			\draw[tuborg, decoration={brace}] let
			    \p1=(G-s.north), \p2=(G-e1) in
					    ($(-1,\y2)$) -- ($(-1,\y1)$) node[tubnode, left]  {Application$\hspace{.3cm}$};
			\draw[tuborg, decoration={brace}] let
			    \p1=(G-e1), \p2=(G-f6.south) in
					    ($(-1,\y2)$) -- ($(-1,\y1)$) node[tubnode, left]  {Framework$\hspace{.3cm}$};

\end{tikzpicture}



==> figures/android-stack.tex <==
%% Android Software Stack

\tikzset{
>=stealth',
  punktchain/.style={
    rectangle, 
    rounded corners, 
    draw=black, very thick,
    text width=10em, 
    text centered, 
    on chain},
  line/.style={draw, thick, <-},
  element/.style={
    tape,
    top color=white,
    bottom color=blue!50!black!60!,
    minimum width=8em,
    draw=blue!40!black!90, very thick,
    text width=10em, 
    text centered, 
    on chain},
  every join/.style={->, thick,shorten >=1pt},
  decoration={brace},
  tuborg/.style={decorate},
  tubnode/.style={midway, right=2pt},
}
\tikzstyle{block} = [draw,fill=white!20,minimum width=4em]
\begin{tikzpicture}
  [node distance=.1cm,
  start chain=going below,]
     \node[punktchain] (applications) {Applications};
				\begin{scope}[start branch=hoejre,]
      		\node (applicationsPl) [block, on chain=going right] {Java};
    		\end{scope}
     \node[punktchain] (framework)      {Framework};
				\begin{scope}[start branch=hoejre,]
      		\node (frameworkPl) [block, on chain=going right] {Java/C/C++};
    		\end{scope}
     \node[punktchain] (libraries)      {Libraries + Dalvik VM};
				\begin{scope}[start branch=hoejre,]
      		\node (librariesPl) [block, on chain=going right] {C/C++};
    		\end{scope}
     \node[punktchain] (kernel) {Kernel};
				\begin{scope}[start branch=hoejre,]
      		\node (kernelPl) [block, on chain=going right] {C};
    		\end{scope}

			\draw[black] let
			    \p1=(kernel.west), \p2=(kernel.east) in
					    ($(\x1-4em,\y1+0.9em)$) -- ($(\x2+4em,\y2+0.9em)$) node[above, midway]  {};
			\draw[tuborg, decoration={brace}] let
			    \p1=(kernel.south), \p2=(kernel.north) in
					    ($(-2,\y1)$) -- ($(-2,\y2)$) node[tubnode, on chain=going left]  {Kernel mode};
			\draw[tuborg, decoration={brace}] let
			    \p1=(libraries.south), \p2=(applications.north) in
					    ($(-2,\y1)$) -- ($(-2,\y2)$) node[tubnode, on chain=going left]  {User mode};

  \end{tikzpicture}


==> figures/android-system-overview.tex <==
%% Android Software Stack

% We need layers to draw the block diagram
\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}

% Define a few styles and constants
\tikzstyle{sensor}=[draw, fill=blue!20, text width=5em, 
    text centered, minimum height=2.5em]
\tikzstyle{ann} = [above, text width=5em]
\tikzstyle{naveqs} = [sensor, text width=6em, fill=red!20, 
    minimum height=12em, rounded corners]

\tikzstyle{zygote} = [draw, fill=white!20, text width=6em, 
	text centered, minimum height=15em]
\tikzstyle{app} = [draw, fill=white!20, text width=6em, 
	text centered, minimum height=15em]
\tikzstyle{systemserver} = [draw, fill=white!20, text width=6em, 
	minimum height=15em]
\tikzstyle{servicemanager} = [draw, fill=white!20, text width=6em, 
	text centered, minimum height=15em]
\tikzstyle{binderdriver} = [draw, fill=white!20, text width=20em, 
	text centered, minimum height=3em, minimum width=24em]
\tikzstyle{service} = [draw, fill=white!20,
	text centered, minimum height=1.4em,  minimum width=14em, rotate=90]
\tikzstyle{stub} = [draw, dashed, rotate=90, minimum height=1.4em, 
	text centered]
\tikzstyle{activity} = [draw, fill=white!20,
	minimum height=13.3em,  minimum width=5em]
\tikzstyle{proxy} = [draw, dashed, rotate=90, minimum height=1.2em, 
	minimum width=1em, text centered]
\def\blockdist{5em}
\def\edgedist{3em}

\begin{tikzpicture}

		%% applications
		\draw (0,0) node (app1) [app, label=above:Applications] {};
		\path (app1)+(-.2em, -.2em) node (app2) [app] {};
		\path (app2)+(-.2em, -.2em) node (app3) [app] {};
		\path (app3)+(-.2em, -.2em) node (app4) [app] {};
			%% activity, services, broadcast receivers, content provider
			\path (app4.south west)+(2.7em,6.85em) node (activity1) [activity, label=above:\small Activity 1.1] {};
				\path (activity1.south west)+(.6em,8.5em) node [minimum width=12em, text width=12em, rotate=90] (mcall1) {\small ...};
				\path (mcall1)+(.9em,0) node [minimum width=12em, text width=12em, rotate=90] (mcall2) {\small am = AccountManager.get();};
				\path (mcall2)+(.9em,0) node [minimum width=12em, text width=12em, rotate=90] (dots) {\small ...};
				\path (dots)+(.9em,0) node [minimum width=12em, text width=12em, rotate=90] (mcall3) {\small am.getAccounts();};
				\path (mcall3)+(.9em,0) node [minimum width=12em, text width=12em, rotate=90] (mcall4) {\small ...};
				%% proxies
				\path (mcall2.west)+(0em,-.9em) node [proxy, text width=1.5em] (mcall2-proxy) {\footnotesize proxy};
				\path (mcall3.west)+(0em,-.9em) node [proxy, text width=1.5em] (mcall3-proxy) {\footnotesize proxy};
		%% service manager
		\path (app1.east)+(+\blockdist,0) node (serviceManager) [servicemanager, label=above:ServiceManager] {};
			\path (serviceManager.south west)+(2.7em,7.25em) node (serviceManagerCode) [activity] {};
				\path (serviceManagerCode.south west)+(.6em,8.5em) node [minimum width=12em, text width=12em, rotate=90] (method1) {\small ...};
				\path (method1)+(.9em,0) node [minimum width=12em, text width=12em, rotate=90] (method2) {\small getService(String) \{ ... \}};
				\path (method2)+(.9em,0) node [minimum width=12em, text width=12em, rotate=90] (method3) {\small ...  };
				\path (method3)+(.9em,0) node [minimum width=12em, text width=12em, rotate=90] (method4) {\small addService(String) \{ ... \} };
			%% stubs
			\path (method2.west)+(0em,-1em) node [stub] (serviceManagerCode-stub) {\small stub};
		%% system server	
		\path (serviceManager.east)+(\blockdist+3em,0) node (systemServer) [systemserver, label=above:SystemServer] {};
			%% services
			\path (systemServer.west)+(1.em,+.2em) node (service1) [service] {\small AccountManagerService}; 
			\path (service1)+(1.6em,0) node (service2) [service] {\small Service 2};
			\path (service2)+(1.6em,0) node (serviceDots) [rotate=90] {\small ...};
			\path (serviceDots)+(1.6em,0) node (serviceN) [service] {\small Service N};
			%% stubs
			\path (service1.west)+(0,1.2em) node [stub] (service1-stub) {stub};
			\path (service2.west)+(0,1.2em) node [stub] (service2-stub) {stub};
			\path (serviceN.west)+(0,1.2em) node [stub] (serviceN-stub) {stub};
		%% binder driver
		\draw (serviceManager.south)+(0,-\blockdist+.35em) node (binderDriver) [binderdriver, label=below:Binder driver] {};

		%% arrows
			%% step 1
			\coordinate[shift={(4em,-4em)}] (c1) at (app4.south east);
			\path [draw, -latex] (mcall2-proxy.west) |- (c1) node[above left]{step 1} -| (serviceManagerCode-stub.west);
			%% step 2
			\coordinate[shift={(5em,-5em)}] (c2) at (app4.south east);
			\path [draw, -latex] (mcall3-proxy.west) |- (c2) node[above right]{step 2} -| (service1-stub.west);
			%% step 3
			\coordinate (cCheck) at (service1.north);
			\coordinate (cCheck2) at (service1.east);
			\coordinate[shift={(0em,-1em)}] (cCheckStart) at (cCheck);
			\coordinate[shift={(0em,-1em)}] (cCheckEnd) at (cCheck2);
			\coordinate[shift={(5em,-5em)}] (c2) at (app4.south east);
			\def\myshift#1{\raisebox{1ex}}
			% permission node
			\node at (cCheckEnd) [fill=green!15,draw,circle,scale=0.8,inner sep=0] (checkNode){ck$_P$};
			\draw [draw=black!75, color=black!75, draw, arrows={-latex}] (cCheckStart) to [bend left=45] node[above left]{step 3} (checkNode);

\end{tikzpicture}


==> figures/framework-application-graph.tex <==
%% Framework Application Graph

\pgfdeclarelayer{background}
\pgfdeclarelayer{foreground}
\pgfsetlayers{background,main,foreground}
\tikzstyle{block} = [draw,fill=white!20,minimum width=4em]
\begin{tikzpicture}
  [node distance=.5cm,
  start chain=going below,]

		  \tikzstyle{vertex}=[circle,fill=black!25,minimum size=14pt,inner sep=0pt]
		  \tikzstyle{vInterface}=[block,fill=black!25,minimum size=14pt,inner sep=0pt]
  		\tikzstyle{tuborg}=[decorate]
  		\tikzstyle{tubnode}=[midway, right=2pt]
			% application nodes
		  \foreach \name/\x/\y in {s/1/0, 2/0/1, 3/1/1, 4/2/1, 5/1/2}
		    \node[vertex] (G-\name) at (\x,-\y/1.2) {$\name$};
			% interface nodes
		  \foreach \name/\x/\y in {i1/0/3, i2/1/3, i3/2/3}
		    \node[vInterface] (G-\name) at (\x,-\y/1.2) {$\name$};
		  \node[vInterface] (G-idots) at (3,-3/1.2) {$...$};
		  \node[vInterface] (G-in) at (4,-3/1.2) {$iN$};
		  \foreach \from/\to in {s/2, s/3, s/i3, 2/i1, 2/3, 3/5, 3/4, 5/2, 5/4, 5/i2}
		    \draw[->] (G-\from) -- (G-\to);
			% framework nodes
		  \foreach \name/\x/\y in {f1/0/4, f2/1/4, f3/2/4, f4/0/5, f5/1/5, f6/0/6, f8/4/4, f9/4/5}
		    \node[vertex] (G-\name) at (\x,-\y/1.2) {$\name$};
		  \foreach \name/\x/\y/\n in {ck/1/6/1, ck/3/5/2}
		    \node[vertex,fill=white] (G-\name\n) at (\x,-\y/1.2) {$\name_\n$};
		  \foreach \from/\to in {i1/f1, i2/f2, i3/f3, f1/f4, f2/f5, f2/f4, f4/f6, f4/ck1, f8/f9, f8/ck2, in/f8} 
		    \draw[->] (G-\from) -- (G-\to);

			% background
		  \node[] (G-00) at (0,0) {};
		  \node[] (G-10) at (2,0) {};
		  \node[] (G-01) at (0,-3/1.2) {};
		  \node[] (G-11) at (2,-3/1.2) {};
		  
			\node[] (G-F00) at (0,-3/1.2) {};
		  \node[] (G-F10) at (4,-3/1.2) {};
		  \node[] (G-F01) at (0,-6/1.2) {};
		  \node[] (G-F11) at (4,-6/1.2) {};
\begin{pgfonlayer}{background}
        % Compute a few helper coordinates
        \path (G-00.west |- G-10.north)+(-0.5,0.3) node (a) {};
        \path (G-01.north -| G-11.east)+(+0.3,-0.1) node (b) {};
        \path[fill=black!5,rounded corners, draw=black!50, dashed]
            (a) rectangle (b);
        \path (G-F00.west |- G-F10.south)+(-0.5,0.1) node (a) {};
        \path (G-F01.south -| G-F11.east)+(+0.3,-0.2) node (b) {};
        \path[fill=black!10,rounded corners, draw=black!50, dashed]
            (a) rectangle (b);
\end{pgfonlayer}

			% naming
			\draw[tuborg, decoration={brace}] let
			    \p1=(G-s.north), \p2=(G-i1) in
					    ($(-1,\y2)$) -- ($(-1,\y1)$) node[tubnode, left]  {Application A$\hspace{.3cm}$};
			\draw[tuborg, decoration={brace}] let
			    \p1=(G-i1), \p2=(G-f6.south) in
					    ($(-1,\y2)$) -- ($(-1,\y1)$) node[tubnode, left]  {Java Framework$\hspace{.3cm}$};

\end{tikzpicture}


